Multi-hop Reading Comprehension through Question Decomposition and Rescoring

Multi-hop Reading Comprehension (RC) requires reasoning and aggregation across several paragraphs. We propose a system for multi-hop RC that decomposes a compositional question into simpler sub-questions that can be answered by off-the-shelf single-hop RC models. Since annotations for such decomposition are expensive, we recast sub-question generation as a span prediction problem and show that our method, trained using only 400 labeled examples, generates sub-questions that are as effective as human-authored sub-questions. We also introduce a new global rescoring approach that considers each decomposition (i.e. the sub-questions and their answers) to select the best final answer, greatly improving overall performance. Our experiments on HotpotQA show that this approach achieves the state-of-the-art results, while providing explainable evidence for its decision making in the form of sub-questions.

==> 03-pipeline.tex <==
We implement a pipeline approach, where a classifier takes a question as a input and outputs the reasoning type. This is different from our decomposition scorer in that the reasoning type is determined in the beginning, before obtaining the answers on all possible reasoning types.

Specifically, we form a sequence of $n$ words, $S$ from the question, obtain $\tilde{S} \in \mathbb{R}^{n \times h}$ from Equation~\ref{eq:bert}, and compute 4-dimensional vector $p_t$ by: \begin{align*} p_t = \mathrm{softmax} (W_3 \mathrm{max}(\tilde{S})) \in \mathbb{R}^4 \end{align*} where $W_3 \in \mathbb{R}^{h \times 4}$ is a parameter matrix. Each element of 4-dimensional vector $p_t$ indicates the reasoning type is bridging, intersection, comparison or original.

==> 10-examples-alg.tex <==
\begin{algorithm*}
\caption{An overall algorithm of \sys{}}\label{alg:overall}
\begin{algorithmic}[1]
\Procedure{\sys}{\text{question}, \text{paragraphs}}
\State $\text{RTs} \gets \{\text{bridging, intersection, comparison, original}\}$
\For{$t$ in $\text{RTs}$}
    \State $\text{answer}_t, \text{evidence}_t \gets  \argmax_{\text{answer, evidence}} P_t (\text{answer, evidence} | \text{question},\text{paragraphs})$
\EndFor
\State $\text{RT}_\text{final} = \argmax_t  P_\text{scorer} (t, \text{answer}_t, \text{evidence}_t|\text{question})$
\State $\text{answer}_\text{final} \gets \text{answer}_{\text{RT}_\text{final}} $
\State \Return $\text{answer}_\text{final}$
\EndProcedure
\end{algorithmic}
\end{algorithm*}


==> 11-model.tex <==
\begin{table*}[tb]
    \centering
    \footnotesize
    \begin{tabular}{l|c|c|c} 
     \toprule
     Model & Single-hop QA & Multi-hop QA & 400 Annotations \\
     \midrule
        Ours & \checkmark & \checkmark & \checkmark \\
        Ours -- No Multi-hop QA Pair & \checkmark &  & \checkmark \\
     \midrule
        \bert~(trained on Multi-hop) & \checkmark & \checkmark &  \\
        \bert~(trained on Single-hop) & \checkmark &  &   \\
     \bottomrule
\end{tabular}
\caption{\hanna{I don't think this table is useful; you can drop it} Four different models, along with the training data. {\em Single-hop QA} indicates the QA pairs from single-hop QA data (\squad{} and \hotpot{} easy), {\em Multi-hop QA} indicates the QA pairs from \hotpot{}, and {\em 400 annotations} indicates the annotations to get spans from the question for decomposition.} 
\label{tab:models}
\vspace{-8pt}
\end{table*}
